Evaluating the Generalization Ability of Quantized LLMs: Benchmark, Analysis, and Toolbox

Large language models (LLMs) have exhibited exciting progress in multiple scenarios, while the huge computational demands hinder their deployments in lots of real-world applications. As an effective means to reduce memory footprint and inference cost, quantization also faces challenges in performance degradation at low bit-widths. Understanding the impact of quantization on LLM capabilities, especially the generalization ability, is crucial. However, the community's main focus remains on the algorithms and models of quantization, with insufficient attention given to whether the quantized models can retain the strong generalization abilities of LLMs. In this work, we fill this gap by providing a comprehensive benchmark suite for this research topic, including an evaluation system, detailed analyses, and a general toolbox. Specifically, based on the dominant pipeline in LLM quantization, we primarily explore the impact of calibration data distribution on the generalization of quantized LLMs and conduct the benchmark using more than 40 datasets within two main scenarios. Based on this benchmark, we conduct extensive experiments with two well-known LLMs (English and Chinese) and four quantization algorithms to investigate this topic in-depth, yielding several counter-intuitive and valuable findings, e.g., models quantized using a calibration set with the same distribution as the test data are not necessarily optimal. Besides, to facilitate future research, we also release a modular-designed toolbox, which decouples the overall pipeline into several separate components, e.g., base LLM module, dataset module, quantizer module, etc. and allows subsequent researchers to easily assemble their methods through a simple configuration. Our benchmark suite is publicly available at https://github.com/TsingmaoAI/MI-optimize

==> chapters/2_framework.tex <==


Besides the common quantization setting, we propose a new perspective to investigate 

We focus on evaluating quantized LLMs, where the quantized models involve an additional quantization phase compared to 
full-precision ones. Hence, we categorize the model evaluation into three stages: pre-training stage, quantization stage, and inference stage (fine-tuning stage and testing stage). Specifically, the pre-training stage corresponds to pre-training data, the quantization stage corresponds to quantization data, the fine-tuning stage in the inference stage corresponds to prompt data, and the testing stage in the inference stage corresponds to testing data. Thus, our framework encompasses four stages of data: pre-training data, quantization (optional), prompt data (optional), and testing data.

\textbf{Pre-training data} typically refers to extensive and diverse datasets comprising various forms of data such as text, images, videos, \textit{etc.}, used to establish the foundational knowledge and understanding capabilities of models~\cite{bert,opt}. These datasets are often sourced from public datasets, web scraping content, or curated data compilations from specific domains. Due to the prohibitively high cost of training a large language model from scratch, the pre-training data in our framework will remain frozen.

\textbf{Quantization data} is used to adjust and optimize the numerical precision of models, ensuring that the model maintains good performance even when running at lower precision levels, such as INT4. In Quantization Aware Training (QAT), pre-trained models are quantized, and then fine-tuning with training data is performed to adjust parameters and recover any precision degradation. In Post-Training Quantization (PTQ), calibration data (\textit{e.g.}, a small subset of training data) is used to compute clipping ranges and scale factors, quantizing the model based on calibration results~\cite{surveyllm,whitepaper,surveyquantization}.

\textbf{Prompt data} is used to elicit and guide the desired behavior from a pre-trained model on specific tasks. When employing large language models, prompt data is typically a series of carefully crafted questions or commands that enable the model to understand and execute particular tasks~\cite{promptmethods,few-shotlearners}. In our framework, prompt data refers to In-context examples of In-context learning.

\textbf{Test data} is utilized to assess the performance of a model on specific tasks. These data should differ from the data used for model pre-training or fine-tuning to ensure the fairness and effectiveness of the evaluation.

The distribution shifts involved in the framework include distribution shifts from quantization data to prompt data, from quantization data to test data, and from prompt data to test data. As addressing all three simultaneously can be complicated, this paper maintains consistency between the distributions of prompt data and test data.


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{figures/评测框架_modified1.pdf}
    \caption{Quantization generalization evaluation framework. Pipelines 1 to 4 maintain consistency between the calibration dataset and the pre-training dataset distribution, aiming to investigate the impact of quantization on the generalization ability of LLM. Pipelines 5 to 8 introduce distribution shift between the calibration dataset and the test dataset, aiming to study the influence of iid calibration dataset and ood calibration dataset on the quantized models.}
\end{figure} 

